Synthetic Data for Social Good

Data for good implies unfettered access to data. But data owners must be conservative about how, when, and why they share data or risk violating the trust of the people they aim to help, losing their funding, or breaking the law. Data sharing agreements can help prevent privacy violations, but require a level of specificity that is premature during preliminary discussions, and can take over a year to establish. We consider the generation and use of synthetic data to facilitate ad hoc collaborations involving sensitive data. A good synthetic dataset has two properties: it is representative of the original data, and it provides strong guarantees about privacy. In this paper, we discuss important use cases for synthetic data that challenge the state of the art in privacy-preserving data generation, and describe DataSynthesizer, a dataset generation tool that takes a sensitive dataset as input and generates a structurally and statistically similar synthetic dataset, with strong privacy guarantees, as output. The data owners need not release their data, while potential collaborators can begin developing models and methods with some confidence that their results will work similarly on the real dataset. The distinguishing feature of DataSynthesizer is its usability - in most cases, the data owner need not specify any parameters to start generating and sharing data safely and effectively. The code implementing DataSynthesizer is publicly available on GitHub at https://github.com/DataResponsibly. The work on DataSynthesizer is part of the Data, Responsibly project, where the goal is to operationalize responsibility in data sharing, integration, analysis and use.

==> ignoreme.tex <==
\julia{This is nice, I made some minor edits to 2 and 3.  I think these can be subsections in vision.tex, maybe rename that section back to ``Use Cases''}

1) Enabling collaboration w/o waiting 18 mos.

introduction has the text

2) Fake linked data

The value of the municipal datasets that motivate our approach enjoy a network effect: each pair of datasets enables new insights. For example, in the City of Seattle, a study is underway to determine the effect of housing instability on high school graduation rates: Do children who endure periods of homelessness graduate on time?  Although the question is simple, it involves linking two extremely sensitive datasets: student data (protected by FERPA and requiring consent of parents to use) and homelessness data (protected by HIPAA and local privacy norms).  In fact, the typical agreements governing the use of these datasets explicitly forbid linking them with any other datasets, and these typical agreements must be revised on a case by case basis to enable such studies.

To bootstrap collaborations over linked data, we might like to use the same approach we have described: generate fake education data, and then generate fake homelessness data.  But this will not work: fake records will not necessarily link with other fake records in a statistically similar was as the real data.  An apparent solution is to simply join the two datasets, then generate a fake dataset from the result.  But this approach entails one data provider sharing their data with another provider, which is explicitly what we need to avoid.

To solve this problem, we want to estimate the statistical properties of the joined dataset, then use that information to guide the data synthesis process independently for the education and homelessness data.

To estimate these properties, we observe that there are three classes of joined tuples: housing records that have no corresponding education records $H$, education records that have no corresponding housing record $E$, and linked pairs of housing and education records $HE$.  We want to estimate the number in each category,  $|H|$,  $|E|$,  $|HE|$. 

To produce these estimates, we can use locality sensitive hashing techniques [LSH] to independently map education tuples and housing tuples into a common space.  Locality sensitive hashing algorithms have the property that similar inputs are mapped to similar outputs, without coordination. For example, integers can be mapped to their most significant $n$ bits.  For structured data, one simple approach is to concatenate the values in the tuples, split this long string into n-grams, sort the n-grams lexicographically, then truncate the sorted list to retain the first $k$ n-grams.  This way, similar tuples will map to similar sequences of n-grams.

Using this approach (or rather, more sophisticated approaches that make use of domain knowledge), we can independently map tuples from different providers into a shared space to determine how likely they are to match, and therefore estimate the counts $|H|$,  $|E|$,  $|HE|$.  Recall that $|H|$ is the number of housing tuples for which no nearby education tuples exist, and $|E|$ is the number of education tuples for which no nearby housing tuples exist.  We can assume the remaining tuples join to produce linked pairs.
Armed with these estimates, we can generate ids for education and housing tuples to ensure that an appropriate number of joined tuples are produced.  Further, we can generate attribute values guided by the same LSH techniques to ensure that joined tuples share similar values.

Applying this approach in a differentially private way remains future work.  

[LSH] https://domino.mpi-inf.mpg.de/intranet/ag5/ag5publ.nsf/0/86BEFB1566020C4AC1257A6400543D05/$file/Nguyen_Master.pdf

3)  Mixing Real and Fake Data

In many data sharing situations, data must be aggregated as an attempt at anonymization.  (Although aggregation approaches offer very little formal protection [x], they are often written into data sharing policies that must be obeyed.)  

For example, energy providers are strongly incentivized to deliver upgrades designed to improve efficiency.  But assessing the efficacy of these upgrades using consumption data, normalized by weather and project specifications, is difficult.  Once again, the problem is to share sensitive data: the energy consumption of customers is a signal-rich resource that could be used for ``cybercasing,'' for example to predict when people leave their homes.  To mitigate such risks, the rules that govern data sharing are designed to prevent disambiguation of aggregate measures.  For instance, a geographic estimate of energy usage must aggregate no fewer than 100 consumers, and no one consumer can represent more than 10\% of the total.  The final calculation must require a certain number of days of recorded usage data. 

We see a novel use case for fake data to ``fill out'' the aggregates to meet anonymity requirements.

Fake data may also be mixed with real data to repair global statistical anomalies, a kind of tuple-level imputation.  For example, one collaborator knows that men between certain ages tend to opt out of registration and data collection activities, resulting in a statistical gap in the data.  This gap can be filled with fake data to help data scientists triage their methods, or obscure the fact that the gap exists, in case data collection activities are sensitive.

4) Adversarial Fake Data Generation



5) Sim city: An fake projection of real city operations.

Related Work: link other papers

http://www.vldb.org/pvldb/vol10/p481-bindschaedler.pdf

https://arxiv.org/pdf/1312.5370.pdf

http://www.ideal.ece.utexas.edu/pubs/pdf/2013/YPark2013.pdf

(same paper I originally sent via ACM)
http://dl.acm.org/citation.cfm?id=2733059


==> scenarios.tex <==
\section{Demonstration Scenario}
\label{sec:scenarios}

\julia{I will restructure or remove this section once the use cases are in place.  Likely the first 2 paragraphs will go into the System section, and the last 2 paragraphs will be dropped once we have usecases.}
\bill{I'd sat remove, or redistribute the important points that aren't made elsewhere.}

We now briefly describe the main components of the \dsspace system. The high-level architecture of the system is presented in Figure~\ref{fig:arch}.  The system has three modules --- \dd, \dgspace and \mi. 
Each component of the system will be explained in detail in Section~\ref{sec:sys}.
A data owner interacts with \dsspace through a Web-based UI that serves as a wrapper for 1) invoking the \ddspace library to compute a data summary, 2) generating a synthetic dataset from the summary using \dg, and 3) inspecting and comparing datasets and data summaries with \mi.

\ddspace can be invoked on any CSV file.  In particular, we can invoke it on both the input file and the output file, and compare the resulting summaries.  Based on this comparison, we will convey an important point to the demonstration attendees: While the input and output datasets themselves are clearly very different, the statistical descriptions of the datasets are very similar.  What sort of a comparison is drawn between the input and the output depends on the mode of operation of \ds.  When the tool in invoked in correlated attribute mode, a comparison of the learned Bayesian networks and of the pair-wise attribute correlations is shown to the user.  In independent attribute mode, per-attribute histograms are presented, along with the ranges of attribute values.

During the demonstration, we will showcase the functionality of \dsspace on a variety of datasets.  We will prepare several interesting datasets for the interactive session, including an urban homelessness dataset from the University of Washington Data Science Institute (where the relevant tasks include making targeted service recommendations), the criminal sentencing dataset from a ProPublica investigation~\cite{propublica} (where the relevant tasks include analyzing the bias of recidivism models), and several datasets from the UCI Machine Learning Repository~\cite{Lichman:2013}. During the demonstration we will encourage users to download additional datasets from portals such as \url{data.seattle.gov} and \url{data.ny.gov} and to run the tool.

Attendees will play the role of a data owner who is preparing a synthetic dataset for release to a set of new collaborators.  After reviewing the raw dataset, they will generate a summary model and inspect the results, verifying that the results are sensible.  Then, the attendees will generate a synthetic dataset from this model and inspect individual records, observing that the records are visibly ``scrambled''.  Finally, they will generate a new model from the synthetic dataset and observe that the statistical properties are intact.  At this point, we will explain the privacy guarantees that are enforced, and will illustrate them using the before-and-after visualizations.





==> system_overview.tex <==
\section{System Overview}
\label{sec:sys}

\julia{We now have a working Web-based UI in addition to Jupyter notebooks.  I'll update this section to include some interesting screenshots.}

\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{figs/architecture.pdf}
	\caption{The \dsspace system architecture.}
 \label{fig:arch}
\end{figure}

\dsspace is an end-to-end system that takes a private dataset as input and generates synthetic datasets. The system is implemented in Python 3.  It assumes that the private dataset is presented in CSV format. 

The input dataset is first processed by the \ddspace module. The domains and the estimates of distributions of the attributes are inferred and saved in a dataset description file. For each attribute identified as categorical, \ddspace computes the frequency distribution of values, represented as a bar chart.  \dgspace then samples from this distribution when deriving the synthetic dataset.  For non-categorical numerical and datetime attributes, \ddspace derives an equi-width histogram to represent the distribution.  \dgspace draws samples from this histogram during data generation using uniform sampling.  For non-categorical string attributes, their minimum and maximum lengths are recorded. \ddspace generates random strings within the length range during data generation stage.

We now describe each of the modules of \dsspace in turn.

\subsection{\dd}

\subsubsection{Inferring data types and domains}

The domain of an attribute is the set of its legal values. The data type is an important ingredient of the attribute domain. \dsspace supports four data types. The system allows users to explicitly specify attribute data types. If an attribute data type is not specified by the user, it is inferred by the \dd. For each attribute, \ddspace first detects whether it is numerical, and if so --- whether it is an \textit{integer} or a \textit{float}. If the attribute is non-numerical, \ddspace attempts to parse it as \textit{datetime}. Any attribute that is neither numerical nor \textit{datetime} is considered a \textit{string}.

\begin{table}
	\centering
    \caption{Data types supported by \ds}
    \label{tab:table_data_types}
    \begin{tabular}{ll}
        \toprule
        Data Type & Example\\
        \midrule
        \textit{integer} & id, age, ... \\
        \textit{float} & score, rating, ... \\
        \textit{string} & name, gender, ... \\
        \textit{datetime} & birthday, event time, ... \\
        \bottomrule
    \end{tabular}
\end{table}

The data type of an attribute restricts its domain, which may be limited further if the attribute is categorical, where only specific values are legal. For example, in a dataset of  students, the attribute \textit{degree} may only take on values  \textit{BS}, \textit{BA}, \textit{MS}, or \textit{PhD}. The domain of \textit{degree} is \{\textit{BS}, \textit{BA}, \textit{MS}, \textit{PhD}\}. Note that \textit{integer}, \textit{float} and \textit{datetime} attributes can also be categorical.  In general, an attribute is considered to be categorical 
if a limited number of distinct values for that attribute is observed in the input dataset.  \ddspace has a parameter \textit{categorical threshold} that defaults to 10 and  represents the maximum number of distinct values for a categorical attribute. 

The {\em categorical threshold}, like any threshold, may be challenging, or even impossible, to set in a way that reflects user preferences for all attributes in the input.  Some attributes may appear categorical, but the user may prefer to treat them as numerical instead.  For example, age of elementary school children may take on only a handful of distinct values but the user may nonetheless wish to generate data for this attribute from a continuous range.  The opposite situation may also arise --- an attribute may take on 200 or so distinct values, as is the case with country names, and so would not be considered categorical under any reasonable threshold.  Still, the user may prefer to treat this attribute as categorical, so that a valid country name, rather than a random string, is generated for this attribute in the synthesized dataset.  For this reason, \dsspace allows users to specify a data type, and state whether an attribute is categorical, over-riding defaults on a per-attribute basis. 

\begin{figure*}[t!]
\centering
\begin{minipage}{3in}
\centering
\includegraphics[width=3in]{figs/AdultIncome_full_age_before.pdf}
\caption{Histogram on \emph{age}: Adult Income~\cite{Lichman:2013}.}
\label{fig:age_before}
\end{minipage}
\begin{minipage}{3.1in}
\centering
\includegraphics[width=3.1in]{figs/AdultIncome_full_age_after.pdf}
\caption{Histogram on \emph{age}: synthetic.}
\label{fig:age_after}
\end{minipage}
\end{figure*}

Note that the actual datatype of a categorical attribute is immaterial in terms of the statistical properties and the privacy guarantees in synthetic data generation.  For example, an attribute such as \textit{sex} may be encoded as {\sf M}/{\sf F}, as {\sf 0}/{\sf 1} or using a Boolean flag (e.g., {\sf True} for male and {\sf False} for female).  In all cases, the tool will compute the frequencies of each attribute value in the input, and will subsequently sample values from the resulting data summary.

There might be missing values in the input dataset, and these are important to represent in the summary. \ddspace calculates the missing rate for each attribute --- the number of observed missing values divided by $n$, the size of the dataset.   

\subsubsection{Differential privacy} \label{sec:diffrential_privacy_implentation}

Differential privacy is a family of techniques that guarantee that the output of an algorithm is statistically indistinguishable on a pair of \emph{neighboring} databases; that is, a pair of databases that differ by only one tuple.  This concept is formalized with the following definition.

($\epsilon$-Differential Privacy~\cite{DBLP:conf/tcc/DworkMNS06})
    Let $\epsilon$ be a positive number. Let $\mathcal{A}$ be a randomized algorithm taking a dataset as input. Let $D$ be a dataset. For any $D'$ that differs from $D$ on at most one tuple, for any legal output $O$ of $\mathcal{A}$, $Pr(\mathcal{A}(D)=O) \leq e^\epsilon \times Pr(\mathcal{A}(D')=O)$.

When $\epsilon$ approaches 0, $Pr(\mathcal{A}(D)=O) = Pr(\mathcal{A}(D')=O)$. That is, the presence or absence of a single individual in the input to the algorithm will be undetectable when one looks at the output.

\subsubsection{Independent attribute mode} \label{sec:unconditioned_distributions}

\begin{figure*}[t!]
\centering
\begin{minipage}{3in}
\centering
\includegraphics[width=3in]{figs/AdultIncome_full_before.pdf}
\caption{Pair-wise correlations: Adult Income~\cite{Lichman:2013}.}
\label{fig:matrix_before}
\end{minipage}
\begin{minipage}{3in}
\centering
\includegraphics[width=3in]{figs/AdultIncome_full_after.pdf}
\caption{Pair-wise correlations: synthetic.}
\label{fig:matrix_after}
\end{minipage}
\end{figure*}

\begin{figure*}[t!]
\centering
\begin{minipage}{3in}
\centering
\includegraphics[width=2.8in]{figs/bn_reduced_before.pdf}
\caption{Bayesian network: Adult Income~\cite{Lichman:2013}.}
\label{fig:bn_before}
\end{minipage}
\begin{minipage}{3in}
\centering
\includegraphics[width=2.8in]{figs/bn_reduced_after.pdf}
\caption{Bayesian network: synthetic.}
\label{fig:bn_after}
\end{minipage}
\end{figure*}

When invoked in independent attribute mode, \ddspace performs frequency-based estimation of the unconditioned probability distributions of the attributes. The distribution is captured by bar charts for categorical attributes, and by histograms for numerical attributes. Precision of the histograms can be refined by a parameter named \textit{histogram size}, which represents the number of bins and is set to 20 by default.

\ddspace implements a differentially private mechanism,  adding controlled noise into the learned distributions. The noise is from a Laplace distribution with location 0 and scale $\frac{1}{n \epsilon}$, where $n$ is the size of the input, denoted $Lap(\frac{1}{n \epsilon})$, setting $\epsilon=0.1$ by default.  \ddspace also adds Laplace noise to the missing rate. When Laplace noise is added to histogram frequencies, the value may become negative.  In that case the value is reset to 0~\cite{DBLP:conf/sigmod/ZhangCPSX14}. 

\subsubsection{Correlated attribute mode} \label{sec:build_Bayesian_networks}

Attribute values are often correlated, e.g., \textit{age} and \textit{income} of a person. When invoked in correlated attribute mode, \ddspace uses the GreedyBayes algorithm to construct Bayesian networks (BN) to model correlated attributes~\cite{DBLP:conf/sigmod/ZhangCPSX14}.

\begin{algorithm}[t!]
	\caption{GreedyBayes($D$, $A$, $k$)}
	\begin{algorithmic}[1]
		\REQUIRE Dataset $D$, set of attributes $A$, maximum number of parents $k$\\
		\STATE Initialize $\mathcal{N}=\emptyset$ and $V=\emptyset$.
		\STATE Randomly select an attribute $X_1$ from $A$.
		\STATE Add $(X_1, \emptyset)$ to $\mathcal{N}$; add $X_1$ to $V$.
		\FOR {$i=2, .., |A|$}
		\STATE Initialize $\Omega = \emptyset$\\
        \STATE $p = min(k, |V|)$\\
		\FOR {each $X \in A \backslash V$ and each $\Pi \in {V \choose p}$}
		\STATE Add $(X, \Pi)$ to $\Omega$
		\ENDFOR
		\STATE Compute mutual information based on $D$ for all pairs in $\Omega$.
		\STATE Select  $(X_i, \Pi_i)$ from $\Omega$ with maximal mutual information.
        \STATE Add $(X_i, \Pi_i)$ to $\mathcal{N}$.
		\ENDFOR
		\RETURN  $\mathcal{N}$
	\end{algorithmic}
	\label{alg:greedy_bayes}
\end{algorithm}

Algorithm \ref{alg:greedy_bayes} constructs a BN $\mathcal{N}$ from input dataset $D$, attributes $A$, and the maximum number of BN node parents $k$, which defaults to 4.  In this algorithm, $V$ is the set of visited attributes, and $\Pi$ is a subset of $V$ that will become parents of node $X$ if added to $\mathcal{N}$. Which attributes $\Pi$ are selected as parents of $X$ is determined greedily, by maximizing  mutual information $(X, \Pi)$. Algorithm \ref{alg:greedy_bayes} learns the structure of the BN with privacy guarantees when the mutual information computation is differentially private ~\cite{DBLP:conf/sigmod/ZhangCPSX14}.

The Bayesian networks constructed in Algorithm \ref{alg:greedy_bayes} gives the sampling order for generating attribute values. The distribution from which a dependent attribute is sampled is called a conditioned distribution.  When constructing noisy conditioned distributions, $Lap(\frac{4(d-k)}{n \cdot \epsilon})$ is injected to preserve privacy.  Here, $d$ is the number of attributes, $k$ is the 
maximum number of parents of a BN node, and $n$ is the number of tuples in the input dataset.  We  construct conditional distributions according to Algorithm 1 of~\cite{DBLP:conf/sigmod/ZhangCPSX14}.

The parents of a dependent attribute can be categorical or numerical, whose distributions are modeled by bar charts and histograms, respectively. The conditions for this dependent attribute are the legal values of the categorical parents and the intervals of the numerical parents. Here, the intervals are formed in the same way as the unconditioned distributions of the parent attributes. For example, the \textit{age} attribute has intervals \{[10, 20),[20, 30),[30, 40)\} in its unconditioned distribution. Assume \textit{education} only depends on \textit{age}. Its conditioned distributions will be under the same intervals, i.e., age $ \in [10,20)$, age $ \in [20,30)$ and age $ \in [30,40)$ respectively.

\subsection{\dg}

Given a dataset description file generated by \dd, \dgspace samples synthetic data from the distributions in this file.  The size of the output dataset is specified by the user, and defaults to $n$, the size of the input dataset. 

\begin{algorithm}[t!]
	\caption{DataGenerator($n, \mathcal{M}, \mathcal{S}, A_U, s$)}
	\begin{algorithmic}[1]
		\REQUIRE number of tuples $n$ to generate, mode $\mathcal{M}$, dataset description $\mathcal{S}$, uniform attributes $A_U$, seed $s$\\
		\STATE Set seed = $s$ for pseudo-random number generator.
		\IF {$\mathcal{M}$ is independent attribute mode}
		\STATE Read all attributes $A$ from $\mathcal{S}$.
        \FOR {$X \in A$}
        \IF {$X \in A_U$}
        \STATE Read the domain of $X$ from $\mathcal{S}$.
        \STATE Sample $n$ values uniformly from its domain.
        \ELSE
        \STATE Read the distribution of $X$ from $\mathcal{S}$.
        \STATE Sample $n$ values from its distribution.
        \ENDIF
        \ENDFOR
        \ELSIF {$\mathcal{M}$ is correlated attribute mode}
        \STATE Read Bayesian network $\mathcal{N}$ from $\mathcal{S}$.
        \STATE Sample root attribute from an unconditional distribution.
        \STATE Sample remaining attributes from conditional distributions. 
        \ENDIF
		\RETURN  Sampled dataset
	\end{algorithmic}
	\label{alg:data_generator}
\end{algorithm}

Algorithm~\ref{alg:data_generator} describes the data generation process.  When invoked in random mode, \dgspace generates  type-consistent random values for each attribute.  When invoked in independent attribute mode, \dgspace draws samples from bar charts or histograms using uniform sampling.  Finally, when invoked in correlated attribute mode, \ddspace samples attribute values in appropriate order from the Bayesian network.

An important property of differential privacy is that its performance degrades with repeated queries. %~\cite{DBLP:conf/uss/HaeberlenPN11}. 
To prevent leaking private information through adversaries repeatedly sending data generation requests, the system administrator can assign a unique random seed for each person who requires a synthetic dataset.  To support this, \dgspace provides per-user seed functionality.

\subsection{Model Inspector}
\label{sec:mi}

\mispace provides several built-in functions to inspect the similarity between the private input dataset and the output synthetic dataset.  The data owner can quickly test whether the tuples in the synthetic dataset are detectable by inspecting and comparing the first 5 and last 5 tuples in both datasets.  

The synthetic dataset should have similar distributions of attribute values as the input dataset. In independent attribute mode, \mispace allows users to visually compare attribute distributions in the form of bar charts or histograms. Figures~\ref{fig:age_before} and~\ref{fig:age_after} present such summaries for the attribute \emph{age} from the Adult Income dataset~\cite{Lichman:2013}. The system also computes the correlation coefficient of an appropriate kind, depending on attribute type, and the KL-divergence value, which measure how much the ``after'' probability distribution diverges from the ``before'' probability distribution for a given attribute.  In correlated attribute mode, \mispace presents ``before'' and ``after'' pairwise mutual information matrices (Figures~\ref{fig:matrix_before} and~\ref{fig:matrix_after}) and describes Bayesian networks (such as those shown graphically in Figures~\ref{fig:bn_before} and~\ref{fig:bn_after}),
enabling an at-a-glance comparison of the statistical properties of the datasets.


